Causal Triplet: An Open Challenge for Intervention-centric Causal Representation Learning

Recent years have seen a surge of interest in learning high-level causal representations from low-level image pairs under interventions. Yet, existing efforts are largely limited to simple synthetic settings that are far away from real-world problems. In this paper, we present Causal Triplet, a causal representation learning benchmark featuring not only visually more complex scenes, but also two crucial desiderata commonly overlooked in previous works: (i) an actionable counterfactual setting, where only certain object-level variables allow for counterfactual observations whereas others do not; (ii) an interventional downstream task with an emphasis on out-of-distribution robustness from the independent causal mechanisms principle. Through extensive experiments, we find that models built with the knowledge of disentangled or object-centric representations significantly outperform their distributed counterparts. However, recent causal representation learning methods still struggle to identify such latent structures, indicating substantial challenges and opportunities for future work. Our code and datasets will be available at https://sites.google.com/view/causaltriplet.

==> figures/graph_old.tex <==
\definecolor{instantcolor}{HTML}{117733} %
\definecolor{edgecolor}{HTML}{444444}

\begin{tikzpicture}
    \centering

    \node (z_1_1) [latent, thick] {$z^1_1$};
    \node (z_1_2) [latent, right=0.2cm of z_1_1, thick] {$z^2_1$};
	\node (z_1_d) [const, right=0.2cm of z_1_2, thick] {$\cdots$} ; %
    \node (z_1_k) [latent, right=0.2cm of z_1_d, thick] {$z^K_1$};

    \plate[inner sep=0.3em,yshift=0.25em,dashed,color=instantcolor, thick] {o1}{(z_1_1) (z_1_2) (z_1_k)}{};
    \node[below right=-12.5pt and -55pt of o1, thick] {$o_1$};

    \node (z_2_1) [latent, right=0.6cm of z_1_k, thick] {$z^1_2$};
    \node (z_2_2) [latent, right=0.2cm of z_2_1, thick] {$z^2_2$};
	\node (z_2_d) [const, right=0.2cm of z_2_2, thick] {$\cdots$}; %
    \node (z_2_k) [latent, right=0.2cm of z_2_d, thick] {$z^K_2$};

    \plate[inner sep=0.3em,yshift=0.25em,dashed,color=instantcolor, thick] {o2}{(z_2_1) (z_2_2) (z_2_k)}{};
    \node[below right=-12.5pt and -55pt of o2, thick] {$o_2$};
    
	\node (o_d) [const, right=0.2cm of o2] {$\cdots$} ; %

    \node (z_3_1) [latent, right=1.2cm of z_2_k, thick] {$z^1_N$};
    \node (z_3_2) [latent, right=0.2cm of z_3_1, thick] {$z^2_N$};
	\node (z_3_d) [const, right=0.2cm of z_3_2, thick] {$\cdots$}; %
    \node (z_3_k) [latent, right=0.2cm of z_3_d, thick] {$z^K_N$};
    
    \plate[inner sep=0.3em,yshift=0.25em,dashed,color=instantcolor, thick] {o3}{(z_3_1) (z_3_2) (z_3_k)}{};
    \node[below right=-12.5pt and -55pt of o3, thick] {$o_N$};

    \node (x) [obs, below=1cm of o2, xshift=-2em, thick] {$x$};

    \edge[color=edgecolor,thick]{o1}{x};
    \edge[color=edgecolor,thick]{o2}{x};
    \edge[color=edgecolor,thick]{o3}{x};
    
    \node (c) [latent, above=1.5cm of o1, xshift=2em, thick] {$c$};
    
    \edge[color=edgecolor,thick]{c}{o1};
    \edge[color=edgecolor,thick]{c}{o2};
    \edge[color=edgecolor,thick]{c}{o3};

    \node (a) [obs, above=of o3, xshift=-4em, thick] {$a$};

    \edge[color=edgecolor,thick]{c}{a};
    \edge[color=edgecolor,thick]{a}{z_3_2};

    \node (z_g) [latent, left=0.8cm of z_1_1, thick] {$z_g$};
    \edge[color=edgecolor,thick]{c}{z_g};

    \path[->, color=edgecolor,thick] (z_g) edge[bend right=20] node[yshift=.5em] {} (x);
    
    % \tikzset{plate caption/.style={caption, node distance=0, inner sep=0pt, text height=1.2em, text depth=0.3em}}
    
\end{tikzpicture}


==> sections/interpretation.tex <==
\subsection{Relation to Causality}
\label{subsec:causal_insights}

% A pair of image observations under intervention can be modeled at different levels of abstractions \citep{rubensteinCausalConsistencyStructural2017a}.

\begin{figure}[t]
    \centering
    \resizebox{0.8\linewidth}{!}{
    \input{figures/graph}
    }
    \caption{
    Causal graph for a pair of scene observations $(x,\Tilde{x})$ before and after an action $a$.
    The data generating process of each raw observation is described by a set of latent factors, including global scene-level factors $z_g$ and local object-level factors $z_n^k$.
    The constituent objects $\{o_1, o_2, \cdots, o_N\}$ are permutation symmetric, and so are the latent factors of each object.
    The action is assumed to sparsely influence only one (or a few) latent factors of an object in the scene.
    The other latent factors may stay constant in photo-realistic simulations but vary over time in real-world observations.
    }
    \label{fig:causal_graph}
\end{figure}

Modeling actions that affect the underlying structure of natural scenes is tied to discovering causal variables and mechanisms from raw observations. Below we provide a brief interpretation of the underlying data generating process from a causal standpoint.

\paragraph{Paired observations as actionable counterfactuals.} 
Several prior works \citep{locatelloWeaklySupervisedDisentanglementCompromises2020a,vonkugelgenSelfSupervisedLearningData2021, brehmerWeaklySupervisedCausal2022} assume having access to pairs of observations that share the majority of the underlying generative factors except the ones under intervention.
The image pairs in this setup can be viewed as a counterfactual, with only a few causal variables being hypothetically intervened from their factual values.
While such data pairs are likely missing in nature in general~\citep{hollandStatisticsCausalInference1986}, they might be in part plausible for embodied agents learning to discover causal models through interactions with the world \citep{cohenGroundedTheoryCausation2022}, \textit{e.g.}, a robot intentionally keeps almost everything unchanged while manipulating an object in the environment, as in our photo-realistic simulations \citep{deitkeProcTHORLargeScaleEmbodied2022}. Of course, this will allow only a subset of all possible counterfactuals, restricting to those that can be realised by the actions of the embodied agent. We call these ``\textit{actionable counterfactuals}''. Unfortunately, even this view would be too restrictive. When it comes to real-world observations, many latent factors may inevitably vary from time to time, \textit{e.g.}, the camera pose $z_g$ changes in our data repurposed from the ego-centric dataset \citep{damenRescalingEgocentricVision2022}, despite being unaffected by the target action. In our setting, we assume that the agent can only perform imperfect actionable counterfactuals, where most objects are not manipulated but the global properties of the visual scene may change. This is a step towards \textit{Intervention Centric Causal Representation Learning}, where \bernhard{interventions are associated with (and represented alongside) with objects, changing an object's dynamics in whenever they take place.}

%all variables can change under their natural dynamic and the intervention changes the dynamic from the prior state. 

\paragraph{Sparse mechanism shifts between visual representations.} 
Given the causal graph in \cref{fig:causal_graph}, the joint distribution of the latent factors can be factorized into causal conditionals,
\begin{equation*}
    p(o_1, o_2, \cdots, o_N, g_z, c) = p(g_z \mid c) \prod_i^N p(o_i \mid c),
\end{equation*}
where only one or a few conditionals changes under intervention \citep{scholkopfCausalRepresentationLearning2021a}.
Intuitively, an action does not manipulate all objects in a scene nor alter all properties of the intervened object at the same time.
Instead, it may sparsely affects a small subset of latent components in a causally structured visual representation space \citep{locatelloWeaklySupervisedDisentanglementCompromises2020a, lachapelleDisentanglementMechanismSparsity2022}.


\paragraph{Independent causal mechanisms for action representations.}

Modeling the effect of an action essentially amounts to learning a causal mechanism $p(\Tilde{z}_n^k \mid z_n^k, a)$, where $z_n^k$ and $\Tilde{z}_n^k$ are the intervened latent factors before and after the action, respectively.
By the Independent Causal Mechanism principle \citep{scholkopfCausalAnticausalLearning2012,petersElementsCausalInference2017}, the conditional distribution of each variable given its causes does not inform or influence the other conditional distributions.
\update{
In other words, the mechanism $p(\Tilde{z}_n^k \mid z_n^k, a)$ is independent of the mechanism generating the action $p(a \mid c)$.
This implies that action representations build upon the former mechanism should remain robust in the presence of distribution shifts on the latter.
}

% This implies that while actions might be statistically correlated with some unintervened object attributes due to known or unknown confounders $c$ (\textit{e.g.}, our compositional data split introduces strong but unstable correlations between the object class and action class), \todo{rewrite} a robust action representation should not capture such non-causal dependencies.

==> sections/model.tex <==

\subsection{Distributed Representations}

TODO

\skeleton{ResNet} \citep{heDeepResidualLearning2016}

\skeleton{Clip} \citep{radfordLearningTransferableVisual2021a}

\subsection{Disentangled Representation of Actions from Objects}

TODO

\skeleton{Adversarial training}

\skeleton{HSIC (todo)}

\citep{atzmonCausalViewCompositional2020,ruisIndependentPrototypePropagation2021}

\subsection{Disentangled Representations of Single-object Images}

TODO

\skeleton{Fully Supervised Disentanglement}

\skeleton{Weakly Supervised Disentanglement}

\citep{locatelloWeaklySupervisedDisentanglementCompromises2020a,lippeCITRISCausalIdentifiability2022}

\subsection{Slot-based Representations of Multi-object Scenes}

TODO

\skeleton{Oracle Slot-based Representations (Instance Mask)}

\skeleton{Learned Slot-based Representations (GroupVIT)}

\citep{xuGroupViTSemanticSegmentation2022a}

We compare models that exploit the learned latent structures with different group matching modules, including (i) global average, (ii) dense matching, (iii) token-based matching followed by either average pooling or max pooling. 

==> sections/task.tex <==
Causal representation learning, which strives to discover and represent high-level causal variables from low-level sensory observations, is a critical component for combining modern representation learning with classical causal modeling~\citep{scholkopfCausalRepresentationLearning2021a}.
Yet, this is a highly challenging and even ill-posed problem in the unsupervised setting, due to limits of i.i.d. observational data and ambiguities in levels of abstractions.
A promising remedy is to exploit independent causal mechanisms~\citep{scholkopfCausalAnticausalLearning2012,parascandoloLearningIndependentCausal2018a} and sparse mechanism shifts~\citep{scholkopfCausalRepresentationLearning2021a} between pairs of observations under intervention.
Significant progress has been made along this line in both the theoretical underpinnings and practical algorithms~ \citep{locatelloWeaklySupervisedDisentanglementCompromises2020a,vonkugelgenSelfSupervisedLearningData2021,lachapelleDisentanglementMechanismSparsity2022,lippeCITRISCausalIdentifiability2022,brehmerWeaklySupervisedCausal2022}.
However, existing efforts are still confined to simple synthetic data sets that are far from real-world problems.
In this work, we aim to bridge this gap by revisiting recent hypotheses and methods in more realistic settings. Beside the much richer visual complexity of high-dimensional data with heavy occlusions, camera motion, ego motion, and visual scenes with multiple objects, we incorporate two key properties.
%\citep{scholkopfCausalityMachineLearning2019,bengioMetaTransferObjectiveLearning2019,huangCausalDiscoveryHeterogeneous2020,scholkopfCausalRepresentationLearning2021a}  I removed these citations, I believe the SMS was explicitly introduced in our 2021 paper. I also added the ICM one with the reference in which Bernhard first introduced it.

\textit{Desideratum 1:} We take the perspective of embodied agents~\citep{cohenGroundedTheoryCausation2022,deitkeRetrospectivesEmbodiedAI2022} acting in the world, blurring the line between interventions and counterfactuals. In fact, we notice that assuming that only one/few variables change as a result of a sparse shift that maintains the noise realization of all other variables is a counterfactual and not a proper intervention. Arguably, {\em perfect counterfactuals} are difficult to observe, and not all variables may allow observable counterfactuals, invalidating the identifiability results of all existing methods~\citep{locatelloWeaklySupervisedDisentanglementCompromises2020a,vonkugelgenSelfSupervisedLearningData2021,klindtNonlinearDisentanglementNatural2022,brehmerWeaklySupervisedCausal2022}\todo{cite all the papers with theory}. Instead, we propose a practical alternative, where only specific variables corresponding to physical and manipulable objects allow for counterfactual observations while others do not (\textit{e.g.}, camera view, self-occlusions, global scene properties that can change over time). We call this setting ``\textit{actionable counterfactuals}'' -- a setting that can naturally emerge in various situations, such as embodied agents learning to discover causal models through active interventions and human-object interactions observed from a first-person camera view. 

% \todo{we notice that the case where only one variable is intervened and everything else stay the same amounts to a counterfactual when factors are independent. Arguably, while for certain variables counterfactuals can be observed, this is not generally true for every variable.} we stress that {\em perfect counterfactuals} --- only one variables is intervened --- are rare in nature.
% The difficulty in collecting such data pairs renders most previous methods for causal representation learning unfeasible in reality.
% To address this, we propose a practical alternative, where \todo{variables for which counterfactuals can be observed correspond to physical objects.} most objects are not manipulated \todo{at the same time} but the global properties of the visual scene may change \todo{when collecting the data before and after the action}.
% We call it ``\textit{actionable counterfactuals}'' -- a setting that can naturally emerge in various situations, such as embodied agents learning to discover causal models through active interventions and human-object interactions observed from a first-person camera view.

\textit{Desideratum 2:} We argue that the notion of causal representation learning should also move beyond identifying underlying causal factors, and more explicitly account for object affordances that support downstream tasks involving interventions and reasoning.
We thus propose a new task modeling high-level actions between image pairs, with a particular emphasis on out-of-distribution robustness from the independent causal mechanisms principle (\textit{i.e.}, if $X\rightarrow Y$, then $P(Y|X)$ remain valid under interventions on $X$).
This task necessitates the discovery of not only causal variables that can be independently manipulated but also causal mechanisms behind actions that govern abstract transformations of object states.
Solving it can be an important step towards \textit{Intervention-Centric Causal Representation Learning}, where interventions are associated with (and represented alongside) objects, changing an object's default dynamics whenever they take place.

In light of these two desiderata, we introduce a new benchmark for causal representation learning, named \causaltriplet. 
It features (i) pairs of images with high visual complexity and variability, (ii) real-world actions inducing sparse changes in the underlying structures of natural scenes.
Through extensive experiments, we show that intervention models built with causally structured representations (\textit{e.g.}, disentangled and object-centric) can substantially outperform distributed representation counterparts on \causaltriplet.
However, recent unsupervised or weakly-supervised methods still have difficulty in correctly discovering the latent structures. In particular, we observe that learning independent causal mechanism is highly challenging in the presence of spurious correlations between actions and object attributes, introducing shortcuts such as recognizing an object based on the action performed or vice-versa that do not generalize to unseen compositions. 
Overall, we hope the proposed benchmark will foster advancement of intervention-centric causal representation learning toward real-world contexts.
% Our code, datasets as well as leaderboard will be made available at URL.

